Time-Varying Poisson Autoregression

In this paper we propose a new time-varying econometric model, called Time-Varying Poisson AutoRegressive with eXogenous covariates (TV-PARX), suited to model and forecast time series of counts. {We show that the score-driven framework is particularly suitable to recover the evolution of time-varying parameters and provides the required flexibility to model and forecast time series of counts characterized by convoluted nonlinear dynamics and structural breaks.} We study the asymptotic properties of the TV-PARX model and prove that, under mild conditions, maximum likelihood estimation (MLE) yields strongly consistent and asymptotically normal parameter estimates. Finite-sample performance and forecasting accuracy are evaluated through Monte Carlo simulations. The empirical usefulness of the time-varying specification of the proposed TV-PARX model is shown by analyzing the number of new daily COVID-19 infections in Italy and the number of corporate defaults in the US.

==> MyDef/def_color.tex <==
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% COLORS
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
\definecolor{darkross}{rgb}{0.008,0.412,0.471}
\definecolor{middleross}{rgb}{0.012,0.580,0.663}
\definecolor{lightross}{rgb}{0.016,0.749,0.855}
\definecolor{darkblue}{rgb}{0.067,0.008,0.471}
\definecolor{middleblue}{rgb}{0.094,0.012,0.663}
\definecolor{lightblue}{rgb}{0.122,0.016,0.855}
\definecolor{darkpurple}{rgb}{0.471,0.008,0.412}
\definecolor{middlepurple}{rgb}{0.663,0.012,0.580}
\definecolor{lightpurple}{rgb}{0.855,0.016,0.749}
\definecolor{darkbrown}{rgb}{0.471,0.067,0.008}
\definecolor{middlebrown}{rgb}{0.663,0.094,0.012}
\definecolor{lightbrown}{rgb}{0.855,0.122,0.016}
\definecolor{darkolive}{rgb}{0.412,0.471,0.008}
\definecolor{middleolive}{rgb}{0.580,0.663,0.012}
\definecolor{lightolive}{rgb}{0.749,0.855,0.016}
\definecolor{darkgreen}{rgb}{0.008,0.417,0.067}
\definecolor{middlegreen}{rgb}{0.012,0.663,0.094}
\definecolor{lightgreen}{rgb}{0.016,0.855,0.122}
\definecolor{darkocre}{rgb}{0.471,0.298,0.008}
\definecolor{middleocre}{rgb}{0.663,0.420,0.012}
\definecolor{lightocre}{rgb}{0.855,0.541,0.016}
%
\def\colorred{\color{red}}
\def\colorblue{\color{middleblue}}
\def\colorgreen{\color{green}}
\def\coloryellow{\color{yellow}}

\def\colordarkross{\color{darkross}}
\def\colordarkblue{\color{darkblue}}
\def\colorlightblue{\color{lightblue}}
\def\colorlightbrown{\color{lightbrown}}
\def\colordarkgreen{\color{darkgreen}}

==> MyDef/def_letters_acc.tex <==
\def\ac{\`a}
\def\ec{\`e}
\def\uc{\`u}
\def\oc{\`o}

\def\acsp{\`a }
\def\ecsp{\`e }
\def\ucsp{\`u }
\def\ocsp{\`o }

\def\qmo{``}
\def\qmc{''}
\def\qmcsp{'' }

==> MyDef/def_letters_b.tex <==
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% LETTERS
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}} 
\def\bi{\mathbf{i}} 
\def\bh{\mathbf{h}}
\def\bp{\mathbf{p}} 
\def\bP{\mathbf{P}}
\def\bff{\mbox{\boldmath $f$}} 
\def\bl{\mbox{\boldmath $l$}}
\def\bJ{\mathbf{J}}
\def\bw{\mathbf{w}}
\def\bL{\mathbf{L}}
\def\br{\mathbf{r}}
\def\bu{\mathbf{u}} 
\def\bt{\mathbf{t}}
\def\by{\mathbf{y}} 
\def\bY{\mathbf{Y}}
\def\0{\mbox{\bf{0}}}
\def\bs{\mathbf{s}}
\def\bS{\mathbf{S}}
\def\bI{\mathbf{I}}
\def\be{\mathbf{e}}
\def\bz{\mathbf{z}}
\def\bZ{\mathbf{Z}}
\def\bC{\mathbf{C}} 
\def\bM{\mathbf{M}}
\def\bc{\mathbf{c}} 
\def\bT{\mathbf{T}}
\def\bW{\mathbf{W}} 
\def\bN{\mathbf{N}} 
\def\bR{\mathbf{R}}
\def\bG{\mathbf{G}} 
\def\bX{\mathbf{X}} 
\def\bx{\mathbf{x}}
\def\bO{\mathbf{0}}
\def\bg{\mathbf{g}}
\def\bv{\mathbf{v}}%
\def\bw{\mathbf{w}}%
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
% CAPITAL LETTERS
% :::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::::
\def\bA{\mathbf{A}}
\def\bE{\mathbf{E}}
\def\bK{\mathbf{K}}
\def\bQ{\mathbf{Q}}
\def\bH{\mathbf{H}}
\def\bF{\mathbf{F}}
\def\bB{\mathbf{B}}
\def\bD{\mathbf{D}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}} 
